User-Network Association in a WLAN-UMTS Hybrid Cell: Global & Individual Optimality

We study optimal user-network association in an integrated 802.11 WLAN and 3G-UMTS hybrid cell. Assuming saturated resource allocation on the downlink of WLAN and UMTS networks and a single QoS class of mobiles arriving at an average location in the hybrid cell, we formulate the problem with two different approaches: Global and Individual optimality. The Globally optimal association is formulated as an SMDP (Semi Markov Decision Process) connection routing decision problem where rewards comprise a financial gain component and an aggregate network throughput component. The corresponding Dynamic Programming equations are solved using Value Iteration method and a stationary optimal policy with neither convex nor concave type switching curve structure is obtained. Threshold type and symmetric switching curves are observed for the analogous homogenous network cases. The Individual optimality is studied under a non-cooperative dynamic game framework with expected service time of a mobile as the decision cost criteria. It is shown that individual optimality in a WLAN-UMTS hybrid cell, results in a threshold policy curve of descending staircase form with increasing Poisson arrival rate of mobiles.

==> figs/hybrid-net.tex <==
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(8396,3860)(2154,-5591)
\put(5626,-4711){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}l}%
}}}}
\put(5776,-4786){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}3G}%
}}}}
\put(5626,-2311){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}l}%
}}}}
\put(5776,-2386){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}AP}%
}}}}
\put(6301,-2311){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}a  \{0,1\}}%
}}}}
\put(6451,-2311){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}e}%
}}}}
\put(6301,-4726){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}a  \{0,2\}}%
}}}}
\put(6451,-4726){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}e}%
}}}}
\put(6976,-3736){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}a  \{0,1,2\}}%
}}}}
\put(7126,-3736){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}e}%
}}}}
\put(8074,-4636){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}   3G}%
}}}}
\put(8074,-4936){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}UMTS}%
}}}}
\put(8074,-5236){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}NodeB}%
}}}}
\thicklines
{\color[rgb]{0,0,0}\put(2176,-2461){\vector( 1, 0){975}}
}%
{\color[rgb]{0,0,0}\put(3406,-5431){\oval(210,210)[bl]}
\put(3406,-2041){\oval(210,210)[tl]}
\put(4996,-5431){\oval(210,210)[br]}
\put(4996,-2041){\oval(210,210)[tr]}
\put(3406,-5536){\line( 1, 0){1590}}
\put(3406,-1936){\line( 1, 0){1590}}
\put(3301,-5431){\line( 0, 1){3390}}
\put(5101,-5431){\line( 0, 1){3390}}
}%
{\color[rgb]{0,0,0}\put(2176,-4861){\vector( 1, 0){975}}
}%
{\color[rgb]{0,0,0}\put(2176,-3661){\vector( 1, 0){975}}
}%
{\color[rgb]{0,0,0}\put(5251,-2461){\vector( 1, 0){2325}}
}%
{\color[rgb]{0,0,0}\put(5251,-4861){\vector( 1, 0){2325}}
}%
{\color[rgb]{0,0,0}\put(5251,-3661){\vector( 1, 0){1425}}
}%
{\color[rgb]{0,0,0}\put(6751,-3736){\vector( 3,-2){986.538}}
}%
{\color[rgb]{0,0,0}\put(6751,-3586){\vector( 3, 2){986.538}}
}%
{\color[rgb]{0,0,0}\put(9226,-2461){\vector( 1, 0){1125}}
}%
{\color[rgb]{0,0,0}\put(9226,-4861){\vector( 1, 0){1125}}
}%
\put(8026,-2536){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}WLAN}%
}}}}
\put(3976,-4186){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}based}%
}}}}
\put(4126,-3436){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}or}%
}}}}
\put(3976,-4636){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}CAC}%
}}}}
\put(3676,-3811){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Interference}%
}}}}
\put(3751,-3061){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Cell Load}%
}}}}
\put(5626,-3511){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}l}%
}}}}
\put(5776,-3586){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}AP,3G}%
}}}}
\put(9376,-2311){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}m}%
}}}}
\put(9526,-2386){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}AP}%
}}}}
\put(9376,-4711){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}l}%
}}}}
\put(9526,-4786){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}AP}%
}}}}
\put(9751,-2311){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(mc)}%
}}}}
\put(9751,-4711){\makebox(0,0)[lb]{\smash{{\SetFigFont{17}{20.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(``eta")}%
}}}}
{\color[rgb]{0,0,0}\put(8401,-2461){\oval(1416,1416)}
}%
{\color[rgb]{0,0,0}\put(8401,-4861){\oval(1416,1416)}
}%
\put(8026,-2836){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}    AP}%
}}}}
\put(8026,-2236){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0} 802.11}%
}}}}
\end{picture}%

